A Formalization of Finite Group Theory: Part III

This is the third and final installment of an exposition of an ACL2 formalization of finite group theory. Part I covers groups and subgroups, cosets, normal subgroups, and quotient groups. Part II extends the theory in the developmnent of group homomorphisms and direct products, which are applied in a proof of the Fundamental Theorem of Finite Abelian Groups. The central topics of the present paper are the symmetric groups and the Sylow theorems, which pertain to subgroups of prime power order. Since these theorems are based on the conjugation of subgroups, an example of a group action on a set, their presentation is preceded by a comprehensive treatment of group actions. Our final result is mainly an application of the Sylow theorems: after showing that the alternating group of order 60 is simple (i.e., has no proper normal subgroup), we prove that no group of non-prime order less than 60 is simple. The combined content of the groups directory is a close approximation to that of an advanced undergraduate course taught by the author in 1976.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{A. Coglio, S. Swords (Eds.): 18th ACL2 Workshop (ACL2-2023)\\
EPTCS 393, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.393.5}{10.4204/EPTCS.393.5}}

